A Framework for Conditional Statement Technical Debt Identification and Description

Technical Debt occurs when development teams favour short-term operability over long-term stability. Since this places software maintainability at risk, technical debt requires early attention to avoid paying for accumulated interest. Most of the existing work focuses on detecting technical debt using code comments, known as Self-Admitted Technical Debt (SATD). However, there are many cases where technical debt instances are not explicitly acknowledged but deeply hidden in the code. In this paper, we propose a framework that caters for the absence of SATD comments in code. Our Self-Admitted Technical Debt Identification and Description (SATDID) framework determines if technical debt should be self-admitted for an input code fragment. If that is the case, SATDID will automatically generate the appropriate descriptive SATD comment that can be attached with the code. While our approach is applicable in principle to any type of code fragments, we focus in this study on technical debt hidden in conditional statements, one of the most TD-carrying parts of code. We explore and evaluate different implementations of SATDID. The evaluation results demonstrate the applicability and effectiveness of our framework over multiple benchmarks. Comparing with the results from the benchmarks, our approach provides at least 21.35%, 59.36%, 31.78%, and 583.33% improvements in terms of Precision, Recall, F-1, and Bleu-4 scores, respectively. In addition, we conduct human evaluation to the SATD comments generated by SATDID. In 1-5 and 0-5 scales for Acceptability and Understandability, the total means achieved by our approach are 3.128 and 3.172, respectively.

==> sections/experiment.tex <==
\section{Experimental Setup}\label{sect:experiment}

...



\subsection{SATD Recommendation}\label{recommend}

In \ac{satd} recommendation, the objective is to build a recommender system. This system will recommend to the developer whether or not they need to write a \ac{satd} comment that self-admits the presence of \ac{td} in a conditional statement.


\subsection{SATD Detection}\label{detect}

...


\subsection{SATD Description}\label{describe}

...


==> sections/rqs.tex <==
\section{Research Questions}\label{sect:rqs}


\subsection{In terms of the dataset,}

\subsubsection{Why are conditional statements interesting?}

\subsubsection{How to prepare and build it for}
\begin{itemize}
    \item Classification
    \item Pre-training
    \item Benchmarking
    \item Comment generation?
\end{itemize}


\subsection{Examining DL,}

\subsubsection{When fine-tuning the SATD recommender, what are the results of the top 5 HP settings}
\begin{itemize}
    \item Without pooling (using the final produced vector)?
    \item With mean-pooling?
    \item With max-pooling?
\end{itemize}

\subsubsection{Using the top 5 HP settings in 10-fold SCV, how effective is LSTM for recommending SATD in conditional statements}
\begin{itemize}
    \item Without pooling?
    \item With mean-pooling?
    \item With max-pooling?
\end{itemize}


\subsection{Examining ML in 10-fold SCV, how effective is MNB, SGD, and TF for recommending SATD in conditional statements}

\subsubsection{With BoWs?}

\subsubsection{With TF-IFD?}


\subsection{Does pre-training help in improving the performance of the recommender system}

\subsubsection{Using end-to-end (fully DL)?}

\subsubsection{Using DL for pre-training and ML for classification?}


\subsection{Benchmarking state-of-the-art approaches}

\subsubsection{Regarding ICSME's paper,}
\begin{itemize}
    \item Can we replicate their approach on our dataset?
    \item How do the results compare with ours?
\end{itemize}

\subsubsection{Regarding EMSE’s paper,}
\begin{itemize}
    \item Can we apply our approach on their dataset?
    \item How do the results compare with theirs?
\end{itemize}


\subsection{Studying generating comments that admit and describe TD found in conditional statements,}

\subsubsection{When fine-tuning, what are the results of 5 different HP settings?}

\subsubsection{Using the best HP setting in 10-fold SCV, how accurate are the generated comments?}

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


